Euclid preparation XXVI. The Euclid Morphology Challenge. Towards structural parameters for billions of galaxies

The various Euclid imaging surveys will become a reference for studies of galaxy morphology by delivering imaging over an unprecedented area of 15 000 square degrees with high spatial resolution. In order to understand the capabilities of measuring morphologies from Euclid-detected galaxies and to help implement measurements in the pipeline, we have conducted the Euclid Morphology Challenge, which we present in two papers. While the companion paper by Merlin et al. focuses on the analysis of photometry, this paper assesses the accuracy of the parametric galaxy morphology measurements in imaging predicted from within the Euclid Wide Survey. We evaluate the performance of five state-of-the-art surface-brightness-fitting codes DeepLeGATo, Galapagos-2, Morfometryka, Profit and SourceXtractor++ on a sample of about 1.5 million simulated galaxies resembling reduced observations with the Euclid VIS and NIR instruments. The simulations include analytic S\'ersic profiles with one and two components, as well as more realistic galaxies generated with neural networks. We find that, despite some code-specific differences, all methods tend to achieve reliable structural measurements (10% scatter on ideal S\'ersic simulations) down to an apparent magnitude of about 23 in one component and 21 in two components, which correspond to a signal-to-noise ratio of approximately 1 and 5 respectively. We also show that when tested on non-analytic profiles, the results are typically degraded by a factor of 3, driven by systematics. We conclude that the Euclid official Data Releases will deliver robust structural parameters for at least 400 million galaxies in the Euclid Wide Survey by the end of the mission. We find that a key factor for explaining the different behaviour of the codes at the faint end is the set of adopted priors for the various structural parameters.

==> double_sersic_table.tex <==
\renewcommand{\arraystretch}{1.8}

\begin{table*}
\centering
\caption{Comparison of the scores $\mathcal{S}$ obtained by the different codes in all structural parameters for the double S\'ersic simulation (with a fixed bulge S\'ersic index fit in red, and with with a free bulge S\'ersic index fit in black). The last column is the mean of the parameters, first for the bulge components and $\mathrm{b/t}$, second for the disk components and $\mathrm{b/t}$. $\texttt{DeepLeGATo}$ is not a model-fitting algorithm, and thus has no fixed or free bulge Sérsic index modes. A smaller $\mathcal{S}$ means a better fit.}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\diagbox{Free bulge fit}{\textcolor{red}{Fix bulge fit}} & $\mathcal{S}_{r_{\rm{e, b}}}$ & $\mathcal{S}_{r_{\rm{e, d}}}$ & $\mathcal{S}_{q_{\mathrm{b}}}$  & $\mathcal{S}_{q_{\mathrm{d}}}$ & $\mathcal{S}_{\rm{b/t}}$ & $\mu_\mathrm{b}, \mu_\mathrm{d}$ \\ 
\hline
~\texttt{DeepLeGATo} & \diagbox{$\emptyset$}{\textcolor{red}{2.42}} & \diagbox{$\emptyset$}{\textcolor{red}{0.49}} & 
\diagbox{$\emptyset$}{\textcolor{red}{0.50}} &
\diagbox{$\emptyset$}{\textcolor{red}{0.21}} &
\diagbox{$\emptyset$}{\textcolor{red}{0.23}} &
\diagbox{$\emptyset$}{\textcolor{red}{1.05 ; 0.31}} \\ 
\hline
\texttt{Galapagos-2} & \diagbox{17.45}{\textcolor{red}{23.13}} &
\diagbox{1.46}{\textcolor{red}{0.91}} &
\diagbox{2.74}{\textcolor{red}{3.50}} &
\diagbox{1.29}{\textcolor{red}{0.51}} &
\diagbox{0.99}{\textcolor{red}{0.95}} &
\diagbox{7.06 ; 1.26}{\textcolor{red}{9.19 ; 0.96}} \\ 
\hline
\texttt{Profit} & \diagbox{37.65}{\textcolor{red}{89.37}} & 
\diagbox{1.37}{\textcolor{red}{1.14}} &
\diagbox{1.92}{\textcolor{red}{1.76}} &
\diagbox{0.60}{\textcolor{red}{0.51}} &
\diagbox{1.22}{\textcolor{red}{1.17}} &
\diagbox{13.6 ; 1.06}{\textcolor{red}{30.76 ; 0.93}} \\ 
\hline
\texttt{SourceXtractor++} & \diagbox{3.00}{\textcolor{red}{3.00}} &
\diagbox{0.51}{\textcolor{red}{0.48}} & 
\diagbox{0.54}{\textcolor{red}{0.53}} &
\diagbox{0.29}{\textcolor{red}{0.29}} &
\diagbox{0.27}{\textcolor{red}{0.26}} &
\diagbox{1.26 ; 0.36}{\textcolor{red}{1.26 ; 0.34}} \\
\hline
\end{tabular}}
\label{table: double sersic}
\end{table*}

==> single_sersic_table.tex <==
\renewcommand{\arraystretch}{1.8}
% \usepackage{diagbox}
% \usepackage{color}


\begin{table}
\caption{Comparison of the scores $\mathcal{S}$ obtained by the different software packages in all structural parameters for the single S\'ersic simulations. Numbers in blue are results from $\textsc{Galsim}$ simulations (discussed in Sec. \ref{sec:ss}), and numbers in black quote results from measurements of simulations with the deep generative model FVAE (discussed in Sec. \ref{sec:real}). The last column is the mean of the parameters. A smaller $\mathcal{S}$ means a better fit.}
\scalebox{0.75}{
\begin{tabular}{|c|c|c|c|c|c} 
\cline{1-5}
\diagbox{FVAE}{\textcolor{blue}{\texttt{Galsim}}} & $\mathcal{S}_{r_{\rm{e}}}$                    & $\mathcal{S}_{\rm{b/a}}$                  & $\mathcal{S}_{\rm{n}}$                    & $\mu_{\mathcal{S}}$                           &   \\ 
\cline{1-5}
DeepLeGATo                               & \diagbox{$\emptyset$}{\textcolor{blue}{0.37}} & \diagbox{$\emptyset$}{\textcolor{blue}{0.25}} & \diagbox{$\emptyset$}{\textcolor{blue}{0.38}} & \diagbox{$\emptyset$}{\textcolor{blue}{0.33}}  &   \\ 
\cline{1-5}
Galapagos-2                              & \diagbox{2.05}{\textcolor{blue}{0.58}}         & \diagbox{0.79}{\textcolor{blue}{0.43}}         & \diagbox{1.29}{\textcolor{blue}{0.60}}        & \diagbox{1.38}{\textcolor{blue}{0.54}}         &   \\ 
\cline{1-5}
Morfometryka                             & \diagbox{$\emptyset$}{\textcolor{blue}{1.10}} & \diagbox{$\emptyset$}{\textcolor{blue}{0.37}} & \diagbox{$\emptyset$}{\textcolor{blue}{1.20}} & \diagbox{$\emptyset$}{\textcolor{blue}{0.89}} &   \\ 
\cline{1-5}
ProFit                                   & \diagbox{1.82}{\textcolor{blue}{0.47}}        & \diagbox{0.65}{\textcolor{blue}{0.21}}        & \diagbox{0.78}{\textcolor{blue}{0.40}}        & \diagbox{1.09}{\textcolor{blue}{0.36}}        &   \\ 
\cline{1-5}
SourceXtractor++                         & \diagbox{1.84}{\textcolor{blue}{0.38}}        & \diagbox{0.60}{\textcolor{blue}{0.18}}        & \diagbox{0.75}{\textcolor{blue}{0.29}}         & \diagbox{1.06}{\textcolor{blue}{0.28}}        &   \\
\cline{1-5}
\end{tabular}}
\label{table: single sersic}
\end{table}
